PRISM Lite: A lightweight model for interactive 3D placenta segmentation in ultrasound

Placenta volume measured from 3D ultrasound (3DUS) images is an important tool for tracking the growth trajectory and is associated with pregnancy outcomes. Manual segmentation is the gold standard, but it is time-consuming and subjective. Although fully automated deep learning algorithms perform well, they do not always yield high-quality results for each case. Interactive segmentation models could address this issue. However, there is limited work on interactive segmentation models for the placenta. Despite their segmentation accuracy, these methods may not be feasible for clinical use as they require relatively large computational power which may be especially prohibitive in low-resource environments, or on mobile devices. In this paper, we propose a lightweight interactive segmentation model aiming for clinical use to interactively segment the placenta from 3DUS images in real-time. The proposed model adopts the segmentation from our fully automated model for initialization and is designed in a human-in-the-loop manner to achieve iterative improvements. The Dice score and normalized surface Dice are used as evaluation metrics. The results show that our model can achieve superior performance in segmentation compared to state-of-the-art models while using significantly fewer parameters. Additionally, the proposed model is much faster for inference and robust to poor initial masks. The code is available at https://github.com/MedICL-VU/PRISM-placenta.

==> text/_1_intro_old.tex <==



\section{INTRODUCTION}
Placental size and shape are associated with adverse perinatal outcomes \cite{biswas2008gross,redman2005latest,schwartz2014first} and fetal size \cite{schwartz2012two}. Accurate volume measurement using 3D ultrasound images (3DUS) is crucial for assessing potential perinatal morbidity and mortality. Although human annotation is the gold standard, it is time-consuming and labor-intensive. Recently, automated segmentation algorithms using Convolutional Neural Networks (CNNs) have shown state-of-the-art performance for placenta segmentation \cite{looney2018fully,looney2021fully,looney2017automatic,oguz2018combining,pouch2020automated,schwartz2022fully,zimmer2023placenta}. However, due to the poor image quality and high levels of noise or artifacts in 3DUS, these methods may not consistently produce robust segmentation for each case. 

Alternatively, interactive segmentation methods could overcome this by using user information to specify the target region. Early work includes the VOCAL platform from GE Healthcare, which utilizes interpolation between manually labeled slices, a random-walker algorithm \cite{STEVENSON20153182}, and a manually initialized multi-atlas label fusion method \cite{oguz2020minimally}. More recently, the Segment Anything Model (SAM) \cite{Kirillov_2023_ICCV} has shown superior performance and wide generalizability for segmentation tasks by taking visual prompts, such as points and boxes. This interactive segmentation model has been widely adopted for medical segmentation tasks \cite{ma2024segment,li2023promise,gong20233dsam,wang2023sam,cheng2023sam,li2024prism,deng2024hats,li2024inter}, including for US applications \cite{yao2023false,lin2023samus,tu2024ultrasound,li2024inter}, to produce robust segmentation. 


As an interactive segmentation model, it should be both effective and efficient in responding to user prompts. Among these SAM-based methods, the PRISM stands out due to its ability to produce segmentations that can reach the human level \cite{li2024prism,li2024inter}. It is designed in a human-in-the-loop manner to mimic human correction behavior to achieve substantial improvements. Moreover, it takes various visual prompts, including points, boxes, scribbles, and masks, to achieve state-of-the-art performance. Its effectiveness and efficiency have been proven through its application in placenta segmentation from 3DUS \cite{li2024inter}. 




Although PRISM has shown state-of-the-art segmentation performance and quick response with provided prompts, its performance can be further improved. A limitation of PRISM is that even though it can accept masks produced from the previous iterations as prompt input to achieve continual improvements, it uses a blank mask for the initial iteration, e.g., starting interactive segmentation from scratch, instead of adapting a binary mask produced from a pretrained model. This contrasts with practical preferred minimally interactive strategies where directly adapting a mask from a pretrained model could improve its efficiency that quickly meets the user expectations. Moreover, It has been demonstrated that using a pretrained foundation model from different imaging modalities \cite{wang2023sam} can improve placenta segmentation performance in 3DUS \cite{li2024inter}, and adapting the masks from pretrained placenta segmentation model may benefit the effectiveness of the PRISM. 




Mobile medical imaging devices, such as portable ultrasound machines, are preferred for point-of-care diagnostics, and lightweight models are desired to meet such clinical demands. However, PRISM, which consists of a hybrid network with transformer and CNN paths as an image encoder, a prompt encoder, and a CNN-based decoder, is not suitable for this purpose as it requires substantial computational resources. Additionally, the large model size slows down its computation speed for real-time applications.


In this paper, we propose a lightweight interactive segmentation model that is designed for clinical application with resource-constrained devices. To achieve efficient and effective performance, we use the framework of the PRISM but modify it to use masks from an automated segmentation model as initialization. To meet the requirements of resource-limited environments, we design the image encoder as a compact model which only has three convolutional blocks. The evaluation is conducted on 3DUS for placenta segmentation. The results indicate that the proposed framework is more effective and efficient for segmenting the placenta. More importantly, it requires less computation resources and has a faster processing speed.





























% Transfer learning is a commonly employed strategy that benefits the initial training phase of a convolutional neural network (CNN) \cite{matsoukas2022makes,mei2022radimagenet,li2024well}. As the availability of publicly accessible medical datasets increases \cite{wang2023sam,wong2023scribbleprompt,li2024well}, it simplifies the training and obtaining of pretrained models for specific tasks or foundational models for various applications. It has been demonstrated that using a pretrained foundation model from different imaging modalities \cite{wang2023sam} can improve placenta segmentation performance in 3DUS \cite{li2024inter}. 




% Thus, adapting the segmentation from pretrained model is important for a robust interactive segmentation model.




% this have led to the development of compact and affordable
% imaging devices that can be used in diverse environment

% mobile medical imaging devices face significant hardware and
% software constraints. Limited processing power, memory, and battery life are major challenges
% that impact the performance of deep learning models. Additionally, the need for real-time
% analysis requires efficient and optimized software capable of delivering accurate results swiftly. 

% Lightweight neural network architectures are designed to be efficient and effective on resourceconstrained devices.


%  to reduce the number of parameters
% and operations.










 
